GenTREC: The First Test Collection Generated by Large Language Models for Evaluating Information Retrieval Systems

Building test collections for Information Retrieval evaluation has traditionally been a resource-intensive and time-consuming task, primarily due to the dependence on manual relevance judgments. While various cost-effective strategies have been explored, the development of such collections remains a significant challenge. In this paper, we present GenTREC , the first test collection constructed entirely from documents generated by a Large Language Model (LLM), eliminating the need for manual relevance judgments. Our approach is based on the assumption that documents generated by an LLM are inherently relevant to the prompts used for their generation. Based on this heuristic, we utilized existing TREC search topics to generate documents. We consider a document relevant only to the prompt that generated it, while other document-topic pairs are treated as non-relevant. To introduce realistic retrieval challenges, we also generated non-relevant documents, ensuring that IR systems are tested against a diverse and robust set of materials. The resulting GenTREC collection comprises 96,196 documents, 300 topics, and 18,964 relevance "judgments". We conducted extensive experiments to evaluate GenTREC in terms of document quality, relevance judgment accuracy, and evaluation reliability. Notably, our findings indicate that the ranking of IR systems using GenTREC is compatible with the evaluations conducted using traditional TREC test collections, particularly for P@100, MAP, and RPrec metrics. Overall, our results show that our proposed approach offers a promising, low-cost alternative for IR evaluation, significantly reducing the burden of building and maintaining future IR evaluation resources.

==> figures/trec_correlation_tabs.tex <==
\begin{figure*}
    \small
    \centering
    \begin{subfigure}{0.4\linewidth}
        \centering
        \begin{tabular}{|c|c|c|c|c|c|c|}
        \hline
        Map & ChatGPT23 & trec5 & trec6 & trec7 & trec8 & robust04 \\ \hline
        ChatGPT23 & 1.0 & 0.51 & 0.69 & 0.78 & 0.82 & 0.73\\ \hline
        trec5 & 0.51 & 1.0 & 0.38 & 0.56 & 0.69 & 0.51\\ \hline
        trec6 & 0.69 & 0.38 & 1.0 & 0.73 & 0.6 & 0.87\\ \hline
        trec7 & 0.78 & 0.56 & 0.73 & 1.0 & 0.78 & 0.87\\ \hline
        trec8 & 0.82 & 0.69 & 0.6 & 0.78 & 1.0 & 0.73\\ \hline
        robust2004 & 0.73 & 0.51 & 0.87 & 0.87 & 0.73 & 1.0\\ \hline
        \textbf{mean} & 0.76 & 0.61 & 0.71 & 0.79 & 0.77 & 0.78\\ \hline
        \end{tabular}
        \caption{Tau correlation between system run results using MAP on TREC collection}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.5\linewidth}
        \centering
        \begin{tabular}{|c|c|c|c|c|c|c|}
        \hline
        Rprec & ChatGPT23 & trec5 & trec6 & trec7 & trec8 & robust04 \\ \hline
        ChatGPT23 & 1.0 & 0.75 & 0.85 & 0.85 & 0.75 & 0.85\\ \hline
        trec5 & 0.75 & 1.0 & 0.67 & 0.76 & 0.84 & 0.76\\ \hline
        trec6 & 0.85 & 0.67 & 1.0 & 0.82 & 0.81 & 0.91\\ \hline
        trec7 & 0.85 & 0.76 & 0.82 & 1.0 & 0.81 & 0.91\\ \hline
        trec8 & 0.75 & 0.84 & 0.81 & 0.81 & 1.0 & 0.9\\ \hline
        robust2004 & 0.85 & 0.76 & 0.91 & 0.91 & 0.9 & 1.0\\
        \hline
        \textbf{mean} & 0.84 & 0.8 & 0.84 & 0.86 & 0.85 & 0.89\\ \hline
        \end{tabular}
        \caption{Tau correlation between system run results using Rprec on TREC collection}
    \end{subfigure}
    
    \bigskip
    \bigskip

    \begin{subfigure}{0.4\linewidth}
        \centering
        \begin{tabular}{|c|c|c|c|c|c|c|}
        \hline
        nDCG & ChatGPT23 & trec5 & trec6 & trec7 & trec8 & robust04 \\ \hline
        chatgpt23 & 1.0 & 0.64 & 0.91 & 0.82 & 0.78 & 0.87\\ \hline
        trec5 & 0.64 & 1.0 & 0.73 & 0.73 & 0.87 & 0.78\\ \hline
        trec6 & 0.91 & 0.73 & 1.0 & 0.91 & 0.87 & 0.96\\ \hline
        trec7 & 0.82 & 0.73 & 0.91 & 1.0 & 0.87 & 0.96\\ \hline
        trec8 & 0.78 & 0.87 & 0.87 & 0.87 & 1.0 & 0.91\\ \hline
        robust2004 & 0.87 & 0.78 & 0.96 & 0.96 & 0.91 & 1.0\\ \hline
        \textbf{mean} & 0.84 & 0.79 & 0.9 & 0.88 & 0.88 & 0.91\\ \hline
        \end{tabular}
        \caption{Tau correlation between system run results using nDCG on TREC collection}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.5\linewidth}
        \centering
        \begin{tabular}{|c|c|c|c|c|c|c|}
        \hline
        P@100 & ChatGPT23 & trec5 & trec6 & trec7 & trec8 & robust04 \\ \hline
        ChatGPT23 & 1.0 & 0.77 & 1.0 & 0.86 & 0.77 & 0.95\\ \hline
        trec5 & 0.77 & 1.0 & 0.77 & 0.81 & 0.91 & 0.81\\ \hline
        trec6 & 1.0 & 0.77 & 1.0 & 0.86 & 0.77 & 0.95\\ \hline
        trec7 & 0.86 & 0.81 & 0.86 & 1.0 & 0.91 & 0.91\\ \hline
        trec8 & 0.77 & 0.91 & 0.77 & 0.91 & 1.0 & 0.81\\ \hline
        robust2004 & 0.95 & 0.81 & 0.95 & 0.91 & 0.81 & 1.0\\ \hline
        \textbf{mean} & 0.89 & 0.85 & 0.89 & 0.89 & 0.86 & 0.9\\ \hline
        \end{tabular}
        \caption{Tau correlation between system run results using P@100 on TREC collection}
    \end{subfigure}
    
    \bigskip
    \bigskip

    \begin{subfigure}{0.4\linewidth}
        \centering
        \begin{tabular}{|c|c|c|c|c|c|c|}
        \hline
        P@10 & ChatGPT23 & trec5 & trec6 & trec7 & trec8 & robust04 \\ \hline
        chatgpt23 & 1.0 & -0.1 & 0.23 & 0.32 & 0.23 & 0.3\\ \hline
        trec5 & -0.1 & 1.0 & 0.71 & 0.61 & 0.66 & 0.63\\ \hline
        trec6 & 0.23 & 0.71 & 1.0 & 0.75 & 0.8 & 0.85\\ \hline
        trec7 & 0.32 & 0.61 & 0.75 & 1.0 & 0.89 & 0.85\\ \hline
        trec8 & 0.23 & 0.66 & 0.8 & 0.89 & 1.0 & 0.94\\ \hline
        robust2004 & 0.3 & 0.63 & 0.85 & 0.85 & 0.94 & 1.0\\ \hline
        \textbf{mean} & 0.33 & 0.58 & 0.72 & 0.74 & 0.75 & 0.76\\ \hline
        \end{tabular}
        \caption{Tau correlation between system run results using P@10 on TREC collection}
    \end{subfigure}
    \caption{Tau correlations between collections}
    \label{fig:trec_correlation_tabs}
\end{figure*}


==> figures/trec_correlation_tabs_colored.tex <==
\newcommand*{\MinNumber}{0.0}%
\newcommand*{\MidNumber}{0.5} %
\newcommand*{\MaxNumber}{1.0}%

%Apply the gradient macro
\newcommand{\ApplyGradient}[1]{%
        \ifdim #1 pt > \MidNumber pt
            \pgfmathsetmacro{\PercentColor}{max(min(100.0*(#1 - \MidNumber)/(\MaxNumber-\MidNumber),100.0),0.00)} %
            \hspace{-0.33em}\colorbox{green!\PercentColor!yellow}{#1}
        \else
            \pgfmathsetmacro{\PercentColor}{max(min(100.0*(\MidNumber - #1)/(\MidNumber-\MinNumber),100.0),0.00)} %
            \hspace{-0.33em}\colorbox{red!\PercentColor!yellow}{#1}
        \fi
}

\newcolumntype{R}{>{\collectcell\ApplyGradient}c<{\endcollectcell}}
\renewcommand{\arraystretch}{0}
\setlength{\fboxsep}{2mm} % box size
\setlength{\tabcolsep}{0pt}

\begin{figure*}
    \small
    \centering
    \begin{subfigure}{0.4\linewidth}
        \centering
        \begin{tabular}{c|*{6}{R}}
        \hline
        %Map & ChatGPT23 & trec5 & trec6 & trec7 & trec8 & robust04 \\ \hline
        chatgpt23 & 1.0 & 0.51 & 0.69 & 0.78 & 0.82 & 0.73\\ \hline
trec5 & 0.51 & 1.0 & 0.38 & 0.56 & 0.69 & 0.51\\ \hline
trec6 & 0.69 & 0.38 & 1.0 & 0.73 & 0.6 & 0.87\\ \hline
trec7 & 0.78 & 0.56 & 0.73 & 1.0 & 0.78 & 0.87\\ \hline
trec8 & 0.82 & 0.69 & 0.6 & 0.78 & 1.0 & 0.73\\ \hline
robust2004 & 0.73 & 0.51 & 0.87 & 0.87 & 0.73 & 1.0\\ \hline
        \end{tabular}
        \caption{Tau correlation between system run results using MAP on TREC collection}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.5\linewidth}
        \centering
        \begin{tabular}{c|*{6}{R}}
        \hline
        %Map & ChatGPT23 & trec5 & trec6 & trec7 & trec8 & robust04 \\ \hline
        chatgpt23 & 1.0 & 0.75 & 0.85 & 0.85 & 0.75 & 0.85\\ \hline
trec5 & 0.75 & 1.0 & 0.67 & 0.76 & 0.84 & 0.76\\ \hline
trec6 & 0.85 & 0.67 & 1.0 & 0.82 & 0.81 & 0.91\\ \hline
trec7 & 0.85 & 0.76 & 0.82 & 1.0 & 0.81 & 0.91\\ \hline
trec8 & 0.75 & 0.84 & 0.81 & 0.81 & 1.0 & 0.9\\ \hline
robust2004 & 0.85 & 0.76 & 0.91 & 0.91 & 0.9 & 1.0\\ \hline
        \end{tabular}
        \caption{Tau correlation between system run results using Rprec on TREC collection}
    \end{subfigure}
    \caption{Tau correlations between collections}
    \label{fig:trec_correlation_tabs}
\end{figure*}


==> figures/trec_correlation_tabs_colored_v2.tex <==
% usage: P{<min>}{<max>}{<siunitx options>}
\newcolumntype{R}[3]{
  >{\collectcell{\colorfromval{#1}{#2}{#3}}} l <{\endcollectcell}}

% #1 = min, #2 = max
% #3 = siunitx options, #4 = cell content
\newcommand*{\colorfromval}[4]{%
  % compute \colorratio in range [0, 100]
  \pgfmathparse{(#4-#1)/(#2-#1)*100}%
  \global\let\colorratio\pgfmathresult
  % set cell color
  \cellcolor{blue!\colorratio}%
  % use command version of column type "S"
  \tablenum[#3]{#4}}


\sisetup{
  round-mode = places,
  round-precision = 3,
  scientific-notation = fixed, 
  fixed-exponent = 0,
  table-format = -1.3
}

\begin{figure*}
    \small
    \centering
    \begin{subfigure}{0.4\linewidth}
        \centering
        \begin{tabular}{l|R{0}{1}{}R{0}{1}{}R{0}{1}{}R{0}{1}{}R{0}{1}{}R{0}{1}{}}
        \hline
        %Map & ChatGPT23 & trec5 & trec6 & trec7 & trec8 & robust04 \\ \hline
        chatgpt23 & 1.0 & 0.51 & 0.69 & 0.78 & 0.82 & 0.73\\ \hline
trec5 & 0.51 & 1.0 & 0.38 & 0.56 & 0.69 & 0.51\\ \hline
trec6 & 0.69 & 0.38 & 1.0 & 0.73 & 0.6 & 0.87\\ \hline
trec7 & 0.78 & 0.56 & 0.73 & 1.0 & 0.78 & 0.87\\ \hline
trec8 & 0.82 & 0.69 & 0.6 & 0.78 & 1.0 & 0.73\\ \hline
robust2004 & 0.73 & 0.51 & 0.87 & 0.87 & 0.73 & 1.0\\ \hline
        \end{tabular}
        \caption{Tau correlation between system run results using MAP on TREC collection}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.5\linewidth}
        \centering
        \begin{tabular}{c|*{6}{c}}
        \hline
        %Map & ChatGPT23 & trec5 & trec6 & trec7 & trec8 & robust04 \\ \hline
        chatgpt23 & 1.0 & 0.75 & 0.85 & 0.85 & 0.75 & 0.85\\ \hline
trec5 & 0.75 & 1.0 & 0.67 & 0.76 & 0.84 & 0.76\\ \hline
trec6 & 0.85 & 0.67 & 1.0 & 0.82 & 0.81 & 0.91\\ \hline
trec7 & 0.85 & 0.76 & 0.82 & 1.0 & 0.81 & 0.91\\ \hline
trec8 & 0.75 & 0.84 & 0.81 & 0.81 & 1.0 & 0.9\\ \hline
robust2004 & 0.85 & 0.76 & 0.91 & 0.91 & 0.9 & 1.0\\ \hline
        \end{tabular}
        \caption{Tau correlation between system run results using Rprec on TREC collection}
    \end{subfigure}
    \caption{Tau correlations between collections}
    \label{fig:trec_correlation_tabs}
\end{figure*}

